(Un)Decidability Bounds of the Synthesis Problem for Petri Games

Petri games are a multi-player game model for the automatic synthesis of distributed systems, where the players are represented as tokens on a Petri net and are grouped into environment players and system players. As long as the players move in independent parts of the net, they do not know of each other; when they synchronize at a joint transition, each player gets informed of the entire causal history of the other players. We show that the synthesis problem for two-player Petri games under a global safety condition is NP-complete and it can be solved within a non-deterministic exponential upper bound in the case of up to 4 players. Furthermore, we show the undecidability of the synthesis problem for Petri games with at least 6 players under a local safety condition.

==> eptcsdata.tex <==
\providecommand{\firstpage}{115}
\providecommand{\publicationstatus}{A. Achilleos and D. Della Monica (Eds.): Fourteenth\\
International Symposium on Games, Automata, Logics,\\
and Formal Verification (GandALF 2023).\\
EPTCS 390, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.390.8}{10.4204/EPTCS.390.8}}


==> sections/0-abstract.tex <==
Petri games are a multi-player game model for the automatic synthesis of
distributed systems,
where the players are represented as tokens on a Petri net and are grouped
into environment players
and system players.
As long as the players move in independent parts of the net, they do not
know of each other;
when they synchronize at a joint transition, each player gets informed
of the
entire causal history of the other players.

We show that the synthesis problem for two-player Petri games under a global safety condition is NP-complete and can be solved within a non-deterministic exponential upper bound in the case of up to 4 players. Furthermore, we show the undecidability of the synthesis problem for Petri games with at least 6 players under a local safety condition. 
%
%\keywords{synthesis,
%	distributed systems,
%	concurrent systems,
%	Petri nets,
%	Petri games,
%	unfolding}
